Dynamic Byzantine-Robust Learning: Adapting to Switching Byzantine Workers

Byzantine-robust learning has emerged as a prominent fault-tolerant distributed machine learning framework. However, most techniques focus on the static setting, wherein the identity of Byzantine workers remains unchanged throughout the learning process. This assumption fails to capture real-world dynamic Byzantine behaviors, which may include intermittent malfunctions or targeted, time-limited attacks. Addressing this limitation, we propose DynaBRO -- a new method capable of withstanding any sub-linear number of identity changes across rounds. Specifically, when the number of such changes is $\mathcal{O}(\sqrt{T})$ (where $T$ is the total number of training rounds), DynaBRO nearly matches the state-of-the-art asymptotic convergence rate of the static setting. Our method utilizes a multi-level Monte Carlo (MLMC) gradient estimation technique applied at the server to robustly aggregated worker updates. By additionally leveraging an adaptive learning rate, we circumvent the need for prior knowledge of the fraction of Byzantine workers.

==> algorithms/dynabro.tex <==
\begin{algorithm}[t]
\caption{\mathodName}\label{alg:method}
\begin{algorithmic}
    \STATE {\bfseries Input:} Initial iterate $x_1\in\reals^d$, learning rates $\cbrac{\eta_t}_{t\geq 1}$. 
    \FOR{$t=1,\ldots,T$}
        \STATE Draw $J_{t} \sim \text{Geom}(\nicefrac{1}{2})$
        % \commentbox{
        % \begin{dottedbox}{Construct gradients}
        \FOR{$k=1,\ldots,2^{J_t}$}
            \FOR{$i\in\sbrac{m}$ in parallel}
                \STATE Compute $g_{t,i}^{k}\gets \nabla F(x_t; \xi_{t,i}^{k})$
                \STATE Send $g_{t,i}^{k}$ if $i\in\G_t^{k}$, else send $*$
            \ENDFOR
        \ENDFOR
        % }
        \FOR{$i\in\sbrac{m}$ in parallel}
            \FOR{$j\in\cbrac{0, J_{t}-1, J_t}$}
                \STATE Compute $\widebar{g}_{t,i}^{j}\gets \frac{1}{2^{j}}\sum_{k=1}^{2^{j}}{g_{t,i}^{k}}$
            \ENDFOR
        \ENDFOR
        % \end{dottedbox}
        \FOR{$j\in\cbrac{0, J_{t}-1, J_t}$}
            \STATE $\widehat{g}_t^{j}\gets \A(\widebar{g}_{t, 1}^{j}, \ldots, \widebar{g}_{t, m}^{j})$ \algorithmiccomment{robust aggregation}
            % \STATE \textbf{Option 2: } $\widehat{g}_t^{j}\gets \text{MFM}(\widebar{g}_{t, 1}^{j}, \ldots, \widebar{g}_{t, m}^{j}; \T^{j})$ \algorithmiccomment{$\T^j=4\V\sqrt{2\log\brac{4m^2 T}/2^{j}}$}
        \ENDFOR
        % \STATE $\Delta_{J_t}\gets 2^{J_t}(\hat{g}_t^{J_{t}} - \hat{g}_t^{J_{t}-1})\mathbbm{1}_{\cbrac{J_t\leq\Jmax}\cap\Ecal_t(J_t)}$
        \STATE $g_t\gets \widehat{g}_t^{0} + \begin{cases} 2^{J_t}(\widehat{g}_t^{J_{t}} - \widehat{g}_t^{J_{t}-1}),& \text{if } \cbrac{{J_t} \leq \Jmax}\cap\Ecal_t \\
        0, & \text{otherwise}.
        \end{cases}$ 
        \algorithmiccomment{$\Ecal_t = \cbrac{\lVert \widehat{g}_t^{J_t} - \widehat{g}_t^{J_t - 1}\rVert\leq 3C_{\nicefrac{1}{mT}}\frac{\V}{\sqrt{2^{J_t}}}\sqrt{\kappa + \frac{2\kappa + 1}{m}}}$} 
        % \STATE \algorithmiccomment{\hspace{-5cm}\textbf{Option 2: } $\Ecal_t = \cbrac{\lVert \widehat{g}_t^{J_t} - \widehat{g}_t^{J_t - 1}\rVert\leq 6C_{\nicefrac{1}{mT}}\frac{\V}{\sqrt{2^{J_t}}}}$}
        % \STATE $\eta_t \gets\eta\cdot\brac{\sum_{\tau=1}^{t}{\lVert g_{\tau}\rVert^2}}^{-1/2}$ \algorithmiccomment{AdaGrad}
        \STATE $x_{t+1}\gets\proj{\K}{x_t - \eta_t g_t}$ 
    \ENDFOR
\end{algorithmic}
\end{algorithm}

==> defs.tex <==
\usepackage[utf8x]{inputenc}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage[round]{natbib}
\usepackage[acronym]{glossaries}
\usepackage[left=2.5cm,right=2.5cm]{geometry}
\usepackage{cancel}
\usepackage[ruled,vlined]{algorithm2e}
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
% \usepackage{algorithm}
\usepackage{algorithmic}
% \usepackage{algpseudocode}
\SetArgSty{textnormal}
\usepackage{graphicx, nicefrac}
\usepackage{subcaption}
\usepackage{booktabs} % To thicken table lines
% \usepackage{algorithm}
\usepackage{comment}
\usepackage{hyperref}
\usepackage[dvipsnames,table,xcdraw]{xcolor}\usepackage{wasysym}
\usepackage{bm} 
\usepackage{multirow}
\usepackage{fancyhdr}
\usepackage{afterpage}
\usepackage{pifont}
\usepackage{cleveref}
\usepackage{thm-restate}
\usepackage{bbm}
\usepackage{enumitem}

\newtheorem{Def}{Definition}
\newtheorem{Thm}{Theorem}
\newtheorem{Lem}{Lemma}
\newtheorem{Fact}{Fact}
\newtheorem{Claim}{Claim}
\newtheorem{Cor}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{Assump}{Assumption}
\renewcommand\theAssump{\arabic{Assump}}


\newcommand{\batchsize}{n}
\newcommand{\threshold}{\T}
\newcommand{\gb}{\bar{g}}


\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}



% \newcommand{\question}[1]{\mycomm{Question}{blue}{#1}}

\newcommand{\RN}[1]{%
  \textup{\uppercase\expandafter{\romannumeral#1}}%
}

% --------------- colors -------------------
\newcommand{\purple}[1]{\textcolor{purple}{#1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{ForestGreen}{#1}}

\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}
% \newcommand{\darkblue}[1]{\textcolor{darkblue}{#1}}
% \definecolor{darkblue}{rgb}{0.0, 0.0, 0.55}

% ------------------------------------------
% --------------- vectors ------------------
\newcommand{\bet}{\boldsymbol{\beta}}
\newcommand{\0}{\boldsymbol{0}}
\newcommand{\Jmax}{\ensuremath{J_{\max}}}

\renewcommand{\a}{\bv{a}}
\renewcommand{\b}{\bv{b}}
\newcommand{\bx}{\bar{\bv{x}}}
\renewcommand{\c}{\bv{c}}
\renewcommand{\d}{\bv{d}}
\newcommand{\e}{\bv{e}}
% \newcommand{\f}{\bv{f}}
\newcommand{\g}{\bv{g}}
\newcommand{\h}{\bv{h}}
\renewcommand{\i}{\bv{i}}
\renewcommand{\j}{\bv{j}}
\renewcommand{\k}{\bv{k}}
\renewcommand{\l}{\bv{l}}
\newcommand{\m}{\bv{m}}
\newcommand{\n}{\bv{n}}
\renewcommand{\o}{\bv{o}}
\newcommand{\p}{\bv{p}}
\newcommand{\q}{\bv{q}}
\renewcommand{\r}{\bv{r}}
\newcommand{\s}{\bv{s}}
% \newcommand{\t}{\bv{t}}
\renewcommand{\u}{\bv{u}}
\renewcommand{\v}{\bv{v}}
\newcommand{\w}{\bv{w}}
\newcommand{\x}{\bv{x}}
\newcommand{\y}{\bv{y}}
\newcommand{\z}{\bv{z}}
\newcommand{\bxi}{\boldsymbol{\xi}}

\newcommand{\xmark}{\text{\ding{55}}}

% ------------------------------------------

% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary}[theorem]
% \newtheorem{lemma}[theorem]{Lemma}

% --------------- commands -----------------
\newcommand{\med}{\text{med}}

\newcommand{\calig}[1]{\mathcal{#1}}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\brac}[1]{\left(#1\right)}
\newcommand{\sbrac}[1]{\left[#1\right]}
\newcommand{\cbrac}[1]{\left\{#1\right\}}
\newcommand{\pbrac}[1]{\left\langle#1\right\rangle}
\newcommand{\expect}[1]{\bb{E}\sbrac{#1}}
\newcommand{\distributed}[2]{#1\sim #2}
\newcommand{\kldiv}[2]{D_{\textup{KL}}(#1\mid\mid#2)}
\newcommand{\MLMC}{\textup{MLMC}}
\newcommand{\nab}{\nabla}
\newcommand{\tv}[2]{D_{\textup{TV}}(#1, #2)}
\newcommand{\dmix}[1]{\textup{d}_\textup{mix}(#1)}
\newcommand{\bbE}{\bb{E}}
\newcommand{\reals}{\bb{R}}
\newcommand{\prob}{\bb{P}}

\newcommand{\errone}{\textup{Err}_1}
\newcommand{\errtwo}{\textup{Err}_2}

\newcommand{\caligS}{\calig{S}}
\newcommand{\caligA}{\calig{A}}
% \newcommand{\caligP}{\calig{P}}
\newcommand{\caligR}{\calig{R}}
\newcommand{\caligM}{\calig{M}}

% ----- Calligraphy Letters ----
\newcommand{\sqd}{\sqrt{D}}
\newcommand{\A}{\calig{A}}
\newcommand{\B}{\calig{B}}
\newcommand{\C}{\calig{C}}
\newcommand{\D}{\calig{D}}
\newcommand{\E}{\calig{E}}
\newcommand{\F}{\calig{F}}
\newcommand{\G}{\calig{G}}
\newcommand{\Hcal}{\calig{H}}
\newcommand{\I}{\calig{I}}
\newcommand{\J}{\calig{J}}
\newcommand{\K}{\calig{K}}
\newcommand{\Lcal}{\calig{L}}
\newcommand{\M}{\calig{M}}
\newcommand{\N}{\calig{N}}
\newcommand{\Ocal}{\calig{O}}
\newcommand{\Ocaltilde}{\tilde{\Ocal}}

\renewcommand{\P}{\calig{P}}
\newcommand{\Q}{\calig{Q}}
\newcommand{\R}{\calig{R}}
\newcommand{\Scal}{\calig{S}}
\newcommand{\T}{\calig{T}}
% \newcommand{\T}{\top}
% \newcommand{\U}{\calig{U}}
\newcommand{\V}{\calig{V}}
\newcommand{\W}{\calig{W}}
\newcommand{\X}{\calig{X}}
\newcommand{\Y}{\calig{Y}}
\newcommand{\Z}{\calig{Z}}

\newcommand{\bv}[1]{\mathbf{#1}}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\proj}[2]{\Pi_{#1}(#2)}
\newcommand{\prox}[2]{\ensuremath{\text{prox}_{#1, #2}}}
% \newcommand{\regret}{\mathrm{Reg}}
\newcommand{\regret}{\mathcal{R}}

\newcommand{\gap}{\texttt{\textup{gap}}}

\newcommand{\diam}{\mathrm{diam}}
\newcommand{\taumix}{\tau_{\mathrm{mix}}}

\newcommand*{\QED}{\null\nobreak\hfill\ensuremath{\blacksquare}}

\newcommand*{\QEDW}{\null\nobreak\hfill\ensuremath{\square}}


\newcommand{\newpar}{\\~\\}

\newcommand{\secref}[1]{Sec.\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\vv}{\ensuremath{\mathbf v}}
\newcommand{\uu}{\ensuremath{\mathbf u}}
\newcommand{\sphere}{\ensuremath{\mathbf S}}

\def\mP{{\mathcal P}}
\def\naturals{{\mathbb N}}
\def\fhat{{\ensuremath{\hat{f}}}}
\def\period{\gamma}

\def\Gtil{\ensuremath{\tilde{G}}}
\def\ptil{\ensuremath{\tilde{p}}}

\newcommand{\df}{\nabla f}
\newcommand{\dF}{\nabla F}
\newcommand{\round}{\mathop{\mbox{\rm round}}}
\newcommand{\myspan}{\mathop{\mbox{\rm span}}}
\newcommand{\edges}{\mathop{\mbox{\rm edges}}}
\newcommand{\conv}{\mathop{\mbox{\rm conv}}}
% \newcommand{\sign}{\mathop{\mbox{\rm sign}}}
\newcommand{\poly}{\mathop{\mbox{\rm poly}}}
\def\Exp{\mathop{\mbox{E}}}
\newcommand{\ignore}[1]{}
\newcommand{\equaldef}{\stackrel{\text{\tiny def}}{=}}
\newcommand{\equaltri}{\triangleq}
\def\trace{{\bf Tr}}
\def\var{{\bf Var}}
\def\reals{{\mathbb R}}
\def\mP{{\mathcal P}}
\def\risk{{\mbox{Risk}}}
\def\ent{{\mbox{ent}}}
\def\mG{{\mathcal G}}
\def\mA{{\mathcal A}}
\def\V{{\mathcal V}}
\def\lhat{\hat{\ell}}
\def\Lhat{\hat{L}}
\def\ltil{\tilde{\ell}}
\def\Ltil{\tilde{L}}

\def\Atil{\tilde{\mathbf{A}}}
\def\Ahat{\hat{\mathbf{A}}}

\def\ball{{\mathbb B}_n}
\def\bold0{\mathbf{0}}
\def\boldone{\mathbf{1}}
\def\boldp{\mathbf{p}}
\def\boldq{\mathbf{q}}
\def\boldr{\mathbf{r}}
\def\boldA{\mathbf{A}}
\def\boldI{\mathbf{I}}
\newcommand\mycases[4] {{
\left\{
\begin{array}{ll}
    {#1} & {#2} \\\\
    {#3} & {#4}
\end{array}
\right. }}
\newcommand\mythreecases[6] {{
\left\{
\begin{array}{ll}
    {#1} & {#2} \\\\
    {#3} & {#4} \\\\
    {#5} & {#6}
\end{array}
\right. }}
% \newcommand\E{\mbox{\bf E}}
% \def\bb{\mathbf{b}}
% \def\bc{\mathbf{c}}
% \def\bB{\mathbf{B}}
% \def\bC{\mathbf{C}}
% \def\be{\mathbf{e}}
% \def\etil{\tilde{\mathbf{e}}}
% \def\bk{\mathbf{k}}
% \def\bu{\mathbf{u}}
% \def\bx{\mathbf{x}}
% \def\w{\mathbf{w}}
% \def\x{\mathbf{x}}
% \def\y{\mathbf{y}}
% \def\z{\mathbf{z}}
% \def\by{\mathbf{y}}
% \def\bz{\mathbf{z}}
% \def\bp{\mathbf{p}}
% \def\bq{\mathbf{q}}
% \def\br{\mathbf{r}}
% \def\bu{\mathbf{u}}
% \def\bv{\mathbf{v}}
% \def\vtil{\tilde{\mathbf{v}}}

\newcommand{\Sp}{\mathbb{S}}

\def\xtil{\tilde{\mathbf{x}}}
\def\xhat{\hat{\mathbf{x}}}
\def\xbar{\bar{\mathbf{x}}}
\def\vol{\mbox{vol}}
\def\trace{{\bf Tr}}
\def\ftil{\tilde{f}}
\def\Exp{\mathop{\mbox{E}}}
\newcommand{\val}{\mathop{\mbox{\rm val}}}
\renewcommand{\deg}{\mathop{\mbox{\rm deg}}}
\newcommand{\eps}{\varepsilon}

\newcommand{\half}{\frac{1}{2}}

\newcommand{\eh}[1]{\textbf{\textcolor{blue}{EH: #1}}}
% \newcommand{\kl}[1]{\textbf{\textcolor{cyan}{KL: #1}}}
\newcommand{\sss}[1]{\textbf{\textcolor{blue}{SSS: #1}}}

\newcommand{\inner}[1]{\langle #1\rangle}


\newcommand{\todo}[1]{\textbf{\textcolor{red}{TODO: #1}}}

\newcommand{\tnabla}{\tilde{\nabla}}


==> sections/main.tex <==
\section{\methodName{}: Dynamic Byzantine-Robustness}\label{sec:dynamic}
% In this section, we turn our focus to the dynamic setting. We demonstrate that a slight modification to \Cref{alg:bro_mlmc} can successfully manage a non-trivial number of ID relabeling rounds (i.e., rounds with Byzantine identity changes). This modification involves adding a fail-safe MLMC filter designed to mitigate any bias a malicious adversary might introduce. Such an adversary may manipulate the Byzantine set by altering identities to exploit the MLMC structure.
In this section, we shift to the dynamic setting, demonstrating how a slightly modified version of \Cref{alg:bro_mlmc} endures non-trivial number of rounds with ID relabeling (i.e., Byzantine identity changes). This modification involves adding a fail-safe MLMC filter, designed to mitigate any bias introduced by a malicious adversary who might manipulate Byzantine identities to exploit the MLMC structure.

% Our MLMC gradient requires each worker to compute a stochastic number of gradients, denoted as $N_t\coloneqq 2^{J_t}$ with $J_t\sim\text{Geom}\brac{1/2}$. To simplify our presentation and analysis, we adopt a modified notation. We denote $\G_{t}^{k}$ as the set of honest workers in round $t\in\sbrac{T}$, specifically when they compute gradients for the $k$-th time, with $k\in\sbrac{N_t}$. In addition, we define $\badrounds\coloneqq\sbrac{T}\setminus\cbrac{t\in\sbrac{T}: \G_{t}^{1}=\cdots=\G_{t}^{N_t}}$ as the set of `bad rounds', where there is a change in the identity of Byzantine workers within that round. Henceforth, we introduce the following constant for ease of writing: 
For our MLMC gradient, each worker computes a stochastic number of gradients, denoted as $N_t\coloneqq 2^{J_t}$ with $J_t\sim\text{Geom}\!\brac{1/2}$. To simplify our presentation and analysis, we adopt a modified notation: Let $\G_{t}^{k}$ represent the set of honest workers in round $t\in\sbrac{T}$, specifically when they compute gradients for the $k$-th time, with $k\in\sbrac{N_t}$. Moreover, we define $\badrounds\coloneqq\sbrac{T}\setminus\cbrac{t\in\sbrac{T}: \G_{t}^{1}=\cdots=\G_{t}^{N_t}}$ as the set of `bad rounds', indicating rounds with changes in Byzantine identities. Henceforth, we introduce the following universal constant for ease of writing: 
\[
    C \coloneqq\sqrt{8 \log{(16m^2 T)}}\; .
\]
\RD{Why/How $\G_t^{k}$ is possible? Isn't sampling fast? -- small batches -- if only between rounds -- no modification is required. Also, if only communications could be altered (what about data poisoning attacks)}

% Given that the MLMC gradient depends solely on $N_t$ computations in round $t$, Byzantine identity changes that occur between rounds do not impact \Cref{alg:bro_mlmc}, ensuring our analysis remains valid. This is also the case for SafeguardSGD~\cite{allen2020byzantine}, which relies on a history window of $T_1\in\O(T^{5/8})$ rounds. However, an omniscient adversary may exploit his knowledge regarding the window size to strategically alter Byzantine identities. 
% To address this in our context, we propose a fail-safe filter specifically designed for the MLMC gradient, as described next. 
Since the MLMC gradient in round $t$ depends solely on $N_t$ computations per-worker in that round, changes in Byzantine identities occurring between rounds do not impact \Cref{alg:bro_mlmc}, ensuring our analysis remains valid. Similar resilience is observed in SafeguardSGD~\cite{allen2020byzantine}, which relies on a history window of $T_1\in\O(T^{5/8})$ rounds. Nevertheless, an omniscient adversary aware of this window size may strategically alter Byzantine identities. To address this in our context, we propose a fail-safe filter designed for the MLMC gradient, detailed as follows. 
\input{algorithms/dynabro_new}

\textbf{MLMC fail-safe filter.} Recall the MLMC gradient formula for $J_t\leq\floor{\log{T}}$, $g_t=\widehat{g}_t^{0} + N_t (\widehat{g}_t^{J_t} - \widehat{g}_t^{J_t-1})$. Its bias and variance analysis hinges on the $c$-LMGO property (\Cref{def:lmgo}) established in \Cref{lem:robust_agg_is_lmgo}, which ensures that for each level $j$, the squared distance between $\widehat{g}_t^{j}$ and $\widehat{g}_t^{j-1}$ decreases as $\O(1/2^{j})$. In good rounds (i.e., without Byzantine identity changes), this property still holds as the set of honest workers is fixed, thus ensuring $\bar{g}_{t,i}^{j}$ and $\bar{g}_{t,i}^{j-1}$ remain honest for all $i\in\G_{t}$.
% Recall that when $J_t\leq \floor{\log{T}}$, the MLMC gradient is given by $g_t=\widehat{g}_t^{0} + N_t (\widehat{g}_t^{J_t} - \widehat{g}_t^{J_t-1})$. The analysis of its bias and variance crucially relies on the $c$-LMGO property (\Cref{def:lmgo}) established in \Cref{lem:robust_agg_is_lmgo}, which ensures that for each level $j$, the squared distance between $\widehat{g}_t^{j}$ and $\widehat{g}_t^{j-1}$ decreases with $j$ as $\O(1/2^{j})$. In `good rounds' $t\in\sbrac{T}\setminus\badrounds$, this property still holds as the set of good workers is fixed within that round and thus $\bar{g}_{t,i}^{j}$ and $\bar{g}_{t,i}^{j-1}$ are honest for every $i\in\G_t$.
% On the other hand, in bad rounds, the method described in \Cref{lem:robust_agg_is_lmgo} is no longer valid as there is no fixed set of honest workers. Since the worker-specific gradient at level $j$, $\bar{g}_{t,i}^j$, is simply an average of messages received from worker $i$, it can be arbitrarily manipulated by even a single Byzantine sample. Therefore, Byzantine machines may collude and arbitrarily switch identities in the second half of each bad round (the last $N_t/2$ samples) to affect most workers and enforce a non-decreasing distance between aggregated gradients at consecutive levels. Accordingly, we define the following event, which simply checks whether this distance is small enough, namely,
Conversely, in bad rounds, the method described in \Cref{lem:robust_agg_is_lmgo} is no longer valid due to the absence of a fixed set of honest workers. For any given worker, the gradient at level $j$, $\bar{g}_{t,i}^j$, is the average of messages that the worker computes in that round. If the worker is compromised by Byzantine behavior even once during that round, this average -- and thus the gradient itself -- can be arbitrarily manipulated by that single Byzantine instance. Byzantine machines can exploit this vulnerability by altering their identities, especially in the second half of a round (the last $N_t/2$ samples), to impact most workers and disrupt the decreasing trend between aggregated gradients at consecutive levels. To counteract this potential manipulation, we introduce an event $\Ecal_t$ to assess whether the gradient distance remains within expected bounds:
\begin{equation}\label{eq:Ecal}
    \Ecal_t = \cbrac{\norm{ \widehat{g}_t^{J_t} - \widehat{g}_t^{J_t - 1}}\leq \frac{(1+\sqrt{2})c_{\Ecal}C\V}{\sqrt{2^{J_t}}}}\; .
\end{equation}

% If $\Ecal_t$ is satisfied, we construct the MLMC estimator as before; otherwise, we use an aggregated gradient based on a single sample per-worker (similarly to when $J_t>\floor{\log{T}}$); see \Cref{alg:method-new} with \textcolor{purple}{\textbf{Option 1}}. Here, $c_{\Ecal}$ is a parameter chosen such that $\Ecal_t$ holds with high probability in good rounds. In such rounds, this modification adds only a lower-order term to the bias bound. In addition, in bad rounds, it ensures that the bias is bounded by only a logarithmic term. 
If $\Ecal_t$ holds, we continue with the standard MLMC construction; otherwise, we default to a simpler aggregated gradient based on a single sample per-worker, similar to the case when $J_t>\floor{\log{T}}$; see \Cref{alg:method-new} with \textcolor{purple}{\textbf{Option 1}}. The parameter $c_{\Ecal}$ is chosen to ensure $\Ecal_t$ holds with high probability in good rounds. In such rounds, this modification adds only a lower-order term to the bias bound, while in bad rounds, it limits the bias to a logarithmic term.


The convergence of our modified algorithm is established in the following theorem, detailed in \Cref{app:dynamic_general}.

\begin{restatable}{theorem}{nonconvex}\label{thm:nonconvex}
    Under \Cref{assump:bounded-noise}, and with a $(\delta, \kappa_{\delta})$-robust aggregator $\A$, consider \Cref{alg:method-new} with \textcolor{purple}{\textbf{Option 1}} and a fixed learning rate given by
    \[
        \eta_t = \eta \coloneqq \min\cbrac{
        \frac{\sqrt{\Delta_1}}{3C\V\sqrt{L\gamma T\log{T}}}, \frac{1}{L}}\; ,
    \]
    where $\gamma\coloneqq 2\kappa_{\delta} + \frac{1}{m}$. Then, the following holds:
    \begin{align*}
        \frac{1}{T}\sum_{t=1}^{T}{\E\!\norm{\nabla_t}^2}&\leq 12C\V\sqrt{\frac{L\Delta_1\gamma\log{T}}{T}}\\  &\hspace{-0.3cm} + \frac{2L\Delta_1 + 9C^2\V^2\gamma}{T} + 16C^2\V^2\gamma\log{T}\frac{\abs{\badrounds}}{T}\; .
    \end{align*}
\end{restatable}

When there are no Byzantine identity switches ($\abs{\badrounds}=0$), we revert to the rate in \Cref{thm:nonconvex-static} for the static setting, but with $\sigma$ effectively replaced by $C\V$ due to differing noise assumptions. 
The bounded noise assumption (\Cref{assump:bounded-noise}) is crucial for two key reasons: First, it ensures that the difference between the aggregated gradient and the true gradient remains bounded, even in bad rounds; second, it allows the application of a concentration inequality, ensuring that $\Ecal_t$ occurs with high probability in good rounds.

\Cref{thm:nonconvex} leads to the subsequent corollary.
\begin{corollary}\label{cor:nonconvex}
    The asymptotic convergence rate implied by \Cref{thm:nonconvex} is given by
    \[
        \frac{1}{T}\sum_{t=1}^{T}{\E\norm{\nabla_t}^2}\in\Otilde\brac{\V\sqrt{\frac{L\Delta_1\gamma}{T}} + \V^2\gamma\frac{\abs{\badrounds}}{T}}\; .
    \]
    Thus, we can handle $\abs{\badrounds}\in\Otilde(\sqrt{T/\gamma})$ bad rounds (omitting the dependence on $L, \Delta_1, $ and $\V$) without affecting the asymptotic convergence rate. Specifically, when $\kappa_{\delta}\in\O(\delta)$, this rate becomes $\Otilde\brac{\V\sqrt{L\Delta_1 (\delta + \nicefrac{1}{m})/T}}$. 
\end{corollary}

\textit{Proof Sketch.}  Following the approach in the proof of \Cref{thm:nonconvex-static}, with $\eta\leq\frac{1}{L}$ we obtain:
\begin{equation*}
    \frac{1}{T}\sum_{t=1}^{T}{\E\!\norm{\nabla_t}^2} \leq \frac{2\Delta_1}{T\eta} + \frac{\eta L}{T}\sum_{t=1}^{T}{\E V_t^2} + \frac{1}{T}\sum_{t=1}^{T}{\E\!\norm{b_t}^2}\; .
\end{equation*}
The bounds for bias and variance are detailed in \Cref{lem:bias-var-mlmc-general}. We highlight key differences from the static setting: in good rounds, the bias is similarly bounded with an additional lower-order term reflecting the instances where $\Ecal_t$ does not hold. In bad rounds, $\Ecal_t$ limits the expected distance between aggregated gradients at consecutive levels as follows:
\begin{align*}
    \E_{t-1}\!\sbrac{\lVert\widehat{g}_t^{j} - \widehat{g}_t^{j-1}\rVert^2\cdot\mathbbm{1}_{\Ecal_t(j)}} &= \\ &\hspace{-10em}\E_{t-1}\sbrac{\lVert{\widehat{g}_t^{j} - \widehat{g}_t^{j-1}}\rVert^2 | \Ecal_t(j)}\prob(\Ecal_t(j))
    \in \Otilde\brac{\frac{\V^2\gamma}{2^{j}}}\; ,
\end{align*}
where $\Ecal_t(j)$ is as defined in \Cref{eq:Ecal} given that $J_t=j$. Taking expectation w.r.t $J_t$ leads to 
\[
    \text{MSE}_t\coloneqq \E_{t-1}\!\norm{g_t - \nabla_t}^2\in\Otilde(\V^2\gamma)\; .
\]
Consequently, the bias is $\Otilde(\V\sqrt{\gamma})$ and the variance for all rounds is $\Otilde(\V^2\gamma)$. To summarize, we have for all $t\in\sbrac{T}$:
\begin{equation*}
    \norm{b_t}\!\in\!\begin{cases}
        \Otilde(\V\sqrt{\gamma}), &t\in\badrounds \\
        \Otilde(\V\sqrt{\frac{\gamma}{T}}), &t\notin\badrounds
    \end{cases}, \hspace{0.4em}\text{and}\hspace{0.4em} V_t^2\!\in\!\Otilde(\V^2\gamma)\; .
\end{equation*}
Substituting these bounds and setting $\eta$ completes the proof. \QEDW

\textbf{When worker momentum fails.} As we elaborate in \Cref{app:momentum_breaks}, the widely-used worker-momentum approach may fail when Byzantine workers change their identities. By meticulously crafting a momentum-tailored \emph{dynamic Byzantine attack} that leverages the momentum parameter and exploits its diminishing weight on past gradients, we can induce a significant drift (i.e., bias) across all worker-momentums, simultaneously. This strategy requires only $\O(\sqrt{T})$ rounds of Byzantine identity changes, which our method can withstand, as shown in \Cref{cor:nonconvex}. Whether it is possible to augment the worker-momentum approach with some mechanism similar to our fail-safe filter, to handle identity changes, remains an intriguing open question.

==> sections/warmup.tex <==
\section{Warm-up: Static Robustness with MLMC}\label{sec:warmup-static}
In this section, we study the static setting where Byzantine machine identities are fixed across time. We develop intuition in \Cref{subsec:motivation}, illustrating how Byzantine machines can hinder convergence. In \Cref{subsec:mlmc_estimation}, we introduce our MLMC estimator, present its bias-variance properties, and highlight its role as a bias reduction technique. Finally, in \Cref{subsec:static-robust}, we show how integrating the MLMC estimator with a robust aggregation rule implies Byzantine-robustness. 
% In this section, we investigate a static setting where Byzantine machine identities are constant over time. We begin by illustrating the impact of Byzantine machines on convergence through bias injection (\Cref{subsec:motivation}). Next, we introduce the Multilevel Monte Carlo (MLMC) estimator, discussing its bias-variance properties and its effectiveness in bias reduction (\Cref{subsec:mlmc_estimation}). We conclude by demonstrating how combining the MLMC estimator with a robust aggregation rule enhances Byzantine robustness (\Cref{subsec:static-robust}).

\subsection{Motivation}\label{subsec:motivation}
% Consider the distributed stochastic gradient descent (D-SGD) update rule, defined for some learning $\eta>0$ as,
% \begin{equation}\label{eq:dsgd}
    % x_{t+1} = x_{t} - \eta \A(g_{t,1},\ldots,g_{t,m})\; ,
% \end{equation}
% where $\A:\reals^{d\times{m}}\to\reals^d$ is some aggregation rule, and $g_{t,i}$ is the message received from worker $i\in\sbrac{m}$ at time $t\in\sbrac{T}$. 
We examine the distributed stochastic gradient descent update rule, defined as $x_{t+1} = x_{t} - \eta \A(g_{t,1},\ldots,g_{t,m})$, with $\eta>0$ as learning rate, $\A:\reals^{d\times{m}}\to\reals^d$ as an aggregation rule, and $g_{t,i}$ representing the message from worker $i\in\sbrac{m}$ at time $t\in\sbrac{T}$. In the Byzantine-free case, $\A$ typically averages the inputs, yet a single Byzantine worker can arbitrarily manipulate this aggregation~\cite{blanchard2017machine}. 

% Ideally, we would expect $\A$ to filter out the Byzantine messages and compute the average of the honest ones, i.e., to output $\widehat{g}_{t} = \frac{1}{\abs{\G}}\sum_{i\in\G}{g_{t,i}}$; this will result is a conditionally unbiased estimate of $\nablat$ with variance reduced by a factor of $\abs{\G}$. However, the Byzantine workers can `hide' within the variance, meaning, they can make themselves indistinguishable from honest workers by sending messages that are within the noise distance from the true gradient, effectively appearing as good~\cite{baruch2019little,xie2020fall,gorbunov2022variance}. Thus, they can inject a bias proportional to the natural noise of the honest workers. For example, if the good messages are within distance $\sigma$ from the true gradient, the Byzantine workers can inject a constant bias of $\O(\sigma\sqrt{\delta})$ in each round, thereby hindering convergence, which will only be possible to a neighborhood of the same order~\cite{ajalloeian2020convergence}.
Ideally, $\A$ would isolate the Byzantine inputs and average the honest inputs, yielding a conditionally unbiased estimate with reduced variance. 
However, Byzantine workers can `blend in' by aligning their messages closely with the expected noise range of honest gradients. Thus, they can inject a bias that is indistinguishable from the natural noise inherent to honest messages, thereby hindering convergence. Specifically, if honest messages deviate by $\sigma$ from the true gradient, Byzantine workers can introduce a bias of $\O(\sigma\sqrt{\delta})$ at each iteration, effectively bounding convergence to a similarly scaled neighborhood~\cite{ajalloeian2020convergence}.

% Building upon the above observation, a naive approach to mitigate the bias introduced by Byzantine workers is to have all honest workers compute stochastic gradients over a large mini-batch, and then employ some robust aggregation rule. Since batching results in variance-reduction, using a large batch size enforces a smaller hiding region for Byzantine workers. Concretely, as we show in \Cref{app:biased-SGD}, theory dictates that using a batch of size $\Omega(T)$ is required to ensure sufficiently low bias. This approach, however, is extremely sample-inefficient, leading to an excessive total of $\Omega(T^2)$ stochastic gradient evaluations per-worker. 
Addressing this challenge, a straightforward mitigation strategy might involve all honest workers computing stochastic gradients across large mini-batches. This approach reduces their variance, thereby shrinking the feasible `hiding region' for Byzantine messages. As we establish in \Cref{app:biased-SGD}, theory suggests a mini-batch size of $\Theta(T)$ is required to ensure sufficiently low bias. However, this approach proves to be extremely inefficient, necessitating an excessive total of $\Theta(T^2)$ stochastic gradient evaluations per worker.  

Instead of implicitly reducing Byzantine bias through honest worker variance reduction, we propose a direct bias reduction strategy by employing an MLMC gradient estimation technique post-aggregation, i.e., to the robustly aggregated gradients. In the next section, we introduce the MLMC estimator and establish its favorable bias-variance properties.

% As an alternative, rather than implicitly reducing Byzantine bias by honest worker variance reduction, we perform direct bias-reduction by employing an MLMC gradient estimation technique post-aggregation, i.e., to the robustly aggregated gradients. The next section outlines the MLMC estimator and its favorable properties, illustrating its ... % In the next section, we present the MLMC estimator and its properties, showing it exhibits a significantly reduced bias compared to the base gradient estimator, at the cost of only logarithmic increase in its variance and the expected number of gradient evaluations.

\subsection{MLMC Gradient Estimation}\label{subsec:mlmc_estimation}
Our MLMC gradient estimator utilizes any method that, given a query vector $x\in\reals^d$ and a budget $N\in\mathbb{N}$ (in terms of stochastic gradient evaluations), produces a vector with a mean squared error (MSE) in estimating $\nabla f(x)$ that is inversely proportional to $N$. Formally, 
\begin{definition}[$c$-LMGO]\label{def:lmgo}
    A mapping $\M_f:\reals^d\times\mathbb{N}\to\reals^d$ is a \emph{linear MSE gradient oracle} (LMGO) of $f$ with constant $c>0$ if for any query $x\in\reals^d$ and budget $N\in\mathbb{N}$, we have:
    \[
        \E\norm{\M_{f}(x, N) - \nabla f(x)}^2\leq \frac{c^2}{N}\; ,
    \]
    where the number of stochastic gradient evaluations of $f$ required for computing $\M_{f}(x, N)$ is at most $N$.
\end{definition}
This definition resembles the \emph{optimal-distance-convergence} method of \citet{asi2021stochastic}; however, our approach bounds the MSE in gradient estimation, whereas they focus on estimating the optimum of strongly-convex functions.

We define the MLMC gradient estimator as follows: 

\vspace{-0.5em}
Sample $J\sim\text{Geom}(\nicefrac{1}{2})$ and, writing $g^{j}\coloneqq \M_{f}(x,2^{j})$, set
\begin{equation}\label{eq:mlmc}
    g^{\text{MLMC}} = g^{0} + \begin{cases}
        2^{J}\brac{g^{J} - g^{J-1}}, &2^J\leq T \\
        0, &\text{otherwise}
    \end{cases}\; .
\end{equation}
The next lemma establishes its properties (cf. \Cref{app:mlmc_bias_reduction}).
\begin{restatable}{lemma}{mlmcprops}\label{lem:mlmc}
    Let $\M_f$ be an \textup{LMGO} of $f$ with constant $c$. For $g^{\textup{MLMC}}$ defined as in \Cref{eq:mlmc}, we have
    \begin{enumerate}
        \item $\textup{Bias}(g^{\textup{MLMC}})\coloneqq\norm{\E g^{\textup{MLMC}} - \nabla f(x)} \leq \sqrt{2c^2/T}$.
        \item $\textup{Var}(g^{\textup{MLMC}})\coloneqq\E\!\norm{g^{\textup{MLMC}} {-} \E g^{\textup{MLMC}}}^2\leq 14c^2\log{T}$.
        \item The expected cost of constructing $g^{\textup{MLMC}}$ is $\O(\log{T})$.
    \end{enumerate}
\end{restatable}
This lemma implies that we can use an LMGO to construct a gradient estimator with: \textbf{(1)} low bias, proportionate to $1/\sqrt{T}$; \textbf{(2)} near-constant variance; and \textbf{(3)} only logarithmic cost in terms of stochastic gradient evaluations.

\subsection{Byzantine-Robustness with MLMC Gradients}\label{subsec:static-robust}
% Next, we demonstrate how integrating the MLMC estimator with a robust aggregation rule ensures Byzantine-resilience. We consider a general family of robust aggregation rules. Concretely, we adopt the notion of $(\delta,\kappa)$-robust aggregator, recently introduced by \citet{allouah2023fixing}, which unifies multiple preceding formulations, e.g., $(f,\lambda)$-resilient averaging~\cite{farhadkhani2022byzantine} and $(\delta_{\max},c)$-\textit{ARAgg}~\cite{karimireddy2022byzantinerobust}.
Next, we show how combining the MLMC estimator with a robust aggregation rule achieves Byzantine-resilience. We consider $(\delta,\kappa_{\delta})$-robust aggregation rules, a concept recently introduced by \citet{allouah2023fixing}, which unifies preceding formulations like $(\delta_{\max},c)$-\textit{RAgg}~\cite{karimireddy2022byzantinerobust}.
\vspace{-1em}
\begin{definition}[$(\delta, \kappa_{\delta})$-robustness]
\label{def:byz-robustness}
Let $\delta< \nicefrac{1}{2}$ and $\kappa_{\delta}\geq 0$. An aggregation rule $\A$ is \textup{$(\delta, \kappa_{\delta})$-robust} if for any vectors $g_1,...,g_m$, and any set $S\subseteq\sbrac{m}$ of size $(1-\delta)m$, we have
\begin{equation*}
    \norm{\A(g_1,\ldots,g_m) - \overline{g}_S}^2\leq \frac{\kappa_\delta}{\abs{S}}\sum_{i\in S}{\norm{g_i - \overline{g}_S}^2}\; ,
\end{equation*}
where $\overline{g}_S = \frac{1}{\abs{S}}\sum_{i\in S}{g_i}$.
\end{definition}
This definition captures, e.g., coordinate-wise median~\cite{yin2018byzantine} and geometric median~\cite{pillutla2022robust}. \RD{CWMed? example for $\kappa_{\delta}$?}

The following lemma demonstrates that applying robust aggregation to mini-batch gradients computed
by honest workers results in a mapping that satisfies \Cref{eq:...} with $c^2=\sigma^2\brac{2\kappa_\delta + \frac{1}{m}}$.
% The following lemma, essential to our analysis, presents a method to construct an LMGO of $f$ using robust aggregation, with honest messages computed over a mini-batch.
% \vspace{-1em}
\begin{restatable}{lemma}{robustagglemmavariance}\label{lem:robust_agg_is_lmgo}
    Consider $x\in\K$ and let $\widebar{g}_1^{\batchsize},\ldots,\widebar{g}_m^{\batchsize}$ be $m$ vectors such that for each $i\in\G$, $\widebar{g}_i^{\batchsize}$ is a mini-batch gradient estimator based on $\batchsize\in\mathbb{N}$ i.i.d samples, i.e., $\widebar{g}_{i}^{\batchsize}\!=\!\frac{1}{\batchsize}\sum_{n=1}^{\batchsize}{\nabla F(x; \xi_{i}^{n})}$, where $\xi_{i}^n\!\overset{\text{i.i.d}}{\sim}\!\D$. Then, under \Cref{assump:bounded-variance}, any $(\delta, \kappa_\delta)$-robust aggregation rule $\A$ satisfies
    \[
        \E\!\norm{\A(\widebar{g}_1^{\batchsize},\ldots,\widebar{g}_m^{\batchsize}) - \nabla f(x)}^2 \leq \frac{\sigma^2}{N}\brac{2\kappa_\delta + \frac{1}{m}}\; .
    \]
\end{restatable}
% \vspace{-0.4em}
% Note that \Cref{lem:robust_agg_is_lmgo}  implies the subsequent result.
\begin{corollary}\label{cor:RA-is-LMGO}
    $\A(\widebar{g}_1^{\batchsize},\ldots,\widebar{g}_m^{\batchsize})$ is an LMGO of $f$ with constant $c^2=\sigma^2\brac{2\kappa_{\delta} + \frac{1}{m}}$.\footnote{Slightly adjusting notation, we extend \Cref{def:lmgo} to the distributed case with a budget of $N$ samples \textbf{per honest worker}.}
\end{corollary}
Building on this result, we propose \Cref{alg:bro_mlmc}. In each round $t\in\sbrac{T}$, we draw $J_t\sim\text{Geom}(\nicefrac{1}{2})$, and each honest worker $i\in\G$ computes three stochastic gradient estimators: $\widebar{g}_{t,i}^{0}$, $\widebar{g}_{t,i}^{J_t-1}$, and $\widebar{g}_{t,i}^{J_t}$, corresponding to mini-batch sizes of $1, 2^{J_t-1}$, and $2^{J_t}$. Robust aggregation is then performed on these estimator groups to derive $\widehat{g}_t^{0}, \widehat{g}_t^{J_t-1}$, and $\widehat{g}_t^{J_t}$, which are used to form the MLMC estimator for the SGD update. 
% Building on this result, we propose \Cref{alg:bro_mlmc}. In each round $t\in\sbrac{T}$, every honest worker $i\in\G$ calculates three stochastic gradient estimators, $\widebar{g}_{t,i}^{0}, \widebar{g}_{t,i}^{J_t-1}$, and $\widebar{g}_{t,i}^{J_t}$ using mini-batches of sizes $1, 2^{J_t-1}$, and $2^{J_t}$, respectively, where $J_t\sim\text{Geom}(\nicefrac{1}{2})$. Subsequently, robust aggregation is applied to each of the three estimators groups to obtain $\widehat{g}_t^{0}$, $\widehat{g}_t^{J_t-1}$, and $\widehat{g}_t^{J_t}$. These estimates are then utilized to construct the MLMC estimator and perform an SGD update.

\input{algorithms/bromag}

The next result confirms the convergence of \Cref{alg:bro_mlmc} for non-convex functions. Its full proof, as well as a convergence statement for the convex case, is deferred to \Cref{app:static-analysis}; here, we provide a proof sketch.
\begin{restatable}{theorem}{nonconvexstatic}\label{thm:nonconvex-static}
    Under \Cref{assump:bounded-variance}, with a $(\delta, \kappa_{\delta})$-robust aggregator $\A$, consider \Cref{alg:bro_mlmc} with learning rate 
    \[
        \eta = \min\cbrac{\frac{\sqrt{\Delta_1}}{3\sigma\sqrt{L\gamma T\log{T}}}, \frac{1}{L}}\; ,
    \]
    where $\gamma\coloneqq 2\kappa_{\delta} + \frac{1}{m}$. Then, for every $T\geq 1$,
    \begin{align*}
        \frac{1}{T}\sum_{t=1}^{T}{\E\!\norm{\nabla_t}^2} &\!\leq\!  12\sqrt{\frac{L\Delta_1\sigma^2 \gamma \log{T}}{T}} + \frac{2\!\brac{L\Delta_1 + \sigma^2 \gamma}}{T}\; .
    \end{align*}
\end{restatable}
% \vspace{-0.5em}
When $\kappa_{\delta}\in\O(\delta)$, e.g., for coordinate-wise median or trimmed mean combined with Nearest Neighbor Mixing~\cite{allouah2023fixing}, the rate in \Cref{thm:nonconvex-static} is consistent with the state-of-the-art convergence guarantees~\cite{karimireddy2021learning,allouah2023fixing}, up to a $\sqrt{\log{T}}$ factor. Moreover, the expected per-worker sample complexity of \Cref{alg:bro_mlmc} is $\O(T\log{T})$, representing a modest increase of only a $\log{T}$ factor over existing methods.

\textit{Proof Sketch.} Consider the following SGD update rule: $x_{t+1} = x_{t} - \eta g_t$, with learning rate $\eta\leq\frac{1}{L}$, and gradients with bias $b_t\coloneqq\E g_t - \nabla_t$ and variance $V_t^2\coloneqq\E\!\norm{g_t - \E g_t}^2$. One can show (cf. \Cref{lem:nonconvex-sgd}) that:
\begin{equation}\label{eq:proof_sketch_nonconvex}
    \frac{1}{T}\sum_{t=1}^{T}{\E\!\norm{\nabla_t}^2} \leq \frac{2\Delta_1}{T\eta} + \frac{\eta L}{T}\sum_{t=1}^{T}{\E V_t^2} + \frac{1}{T}\sum_{t=1}^{T}{\E\!\norm{b_t}^2}\; .
\end{equation}
Combining \Cref{cor:RA-is-LMGO} with \Cref{lem:mlmc} implies that:
\begin{equation}\label{eq:bias-var-static-proofsketch}
    \norm{b_t} \!\leq\! \sqrt{\frac{2\sigma^2\gamma}{T}}, \hspace{0.4em}\text{and}\hspace{0.4em} V_t^2\leq 14\sigma^2\gamma\log{T}, \enskip\forall t\in\sbrac{T} .
\end{equation}
Plugging these bounds and tuning $\eta$ concludes the proof. \QEDW
